Only distances are required to reconstruct submanifolds

In this paper, we give the first algorithm that outputs a faithful reconstruction of a submanifold of Euclidean space without maintaining or even constructing complicated data structures such as Voronoi diagrams or Delaunay complexes. Our algorithm uses the witness complex and relies on the stability of power protection, a notion introduced in this paper. The complexity of the algorithm depends exponentially on the intrinsic dimension of the manifold, rather than the dimension of ambient space, and linearly on the dimension of the ambient space. Another interesting feature of this work is that no explicit coordinates of the points in the point sample is needed. The algorithm only needs the distance matrix as input, i.e., only distance between points in the point sample as input.

==> isaac-manifold-background.tex <==


\section{Manifolds}
\label{sec-manifolds-reach-properties}




% Let $\pi : \R ^d \rightarrow \M$ map each point of $\R ^d$ 
% to its closest point on $\M$. The {\em reach}
% of $\M$, denoted by $\reach$, is defined as the supremum of 
% all $\delta$ such that any point $x$ of $\R ^d$
% lying at distance less than $\delta$ from $\M$ has a unique 
% image $\pi (x)$. In this paper, we assume that
% $\M$ has strictly positive reach. The reach is used for 
% defining sampling conditions on the manifold.




Federer~\cite{federer} proved, $\reach$ is (strictly) positive 
when $\M$ is of class $C^2$ or even $C^{1,1}$, i.e. the normal 
bundle is defined everywhere on $\M$ and is Lipschitz continuous. 
For simplicity, we will assume that $\M$ is a smooth manifold.

%Set $A \subseteq \M$ is called {\em strongly convex} if for any $p,\,q \in A$ there exists a geodesic path
%$\gamma_{pq}\subseteq \M$ such that $\gamma_{pq}$ is the unique minimizer in $\M$
%connecting $p$ to $q$, and $\gamma_{pq}$ is the only geodesic contained in $A$ joining $p$ to $q$.
%Geodesic distance between points $p, \, q \in \M$, denoted by $\|p-q\|_{\M}$, is $\inf_{\gamma_{pq}} |\gamma_{pq}|$
%where $\gamma_{pq}$ is a geodesic connecting $p,\, q$ and $|\gamma_{pq}|$ denotes the length of the geodesic curve.
%Geodesic ball at a point $p \in \M$, denoted by $B_{\rm g}(p,r)$, is defined as
%$$ B_{\rm g}(p,q) := \{q \, : \, \|p-q\|_{\M} \leq r \}.$$
%For a given point $p \in \M$,
%$$r^c(p) = \sup\,\{\,r \,|\, B_{\rm g}(p,r)~\mbox{is strongly convex}\,\}.$$
%The convexity radius of $\M$, denoted by $r^c(\M)$, is
%$$r^c(\M) = \sup_{p\in \M}\, \{\,r^c(p)\,|\,p\in\M\,\}.$$




%\paragraph{$t$-sample}
%A point sample $\pp$ is said to be a {\em $t$-sample} if, for any point $x \in \M$, there exists a point $p\in \pp$ such that
%$\|p-x\| \leq t \,\rch(\M)$.

%We call {\em minimal interpoint distance}  of $\pp$ the smallest distance between any two points of $\pp$. An $\e$-sample
%$\pp$ is called $\kappa$-{\em sparse} if the minimal interpoint distance of $\pp$ is at least $\kappa \, \rch (\M)$.  A
%$\kappa$-sparse $t$-sample of $\M$ is simply called a $(t,\kappa)$-sample.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


We will use the following results 
from~\cite{federer,giesen2004,boissonnat2012con.intrinsic}. 
See~\cite[Lem.~6 \& 7]{giesen2004} 
and~\cite[Lem.~B.3]{boissonnat2012con.intrinsic}.

\begin{lem}\label{lem-sampling-property-manifold}
    Let $p$ and $q$ be points on the manifold $\M$.
    \begin{enumerate}
        \item[1.]
            If $\|p-q\| < \reach$,
%            For all $p, \, q \in \M$ with $\|p-q\| < \reach$,
            $\sin \angle (T_{p}\M, [p \, q]) \leq \frac{\|p-q\|}{2\reach}$.
    \end{enumerate}
    If $\|p-q\| < \frac{\reach}{4}$, then
    \begin{enumerate}
        \item[2.]
            $\dist{q}{\M} \leq \frac{2\|p-q\|^{2}}{\reach}$, and

        \item[3.]
            $\sin \angle(T_{p}\M, T_{q}\M) < \frac{6\|x-y\|}{\reach}$.
    \end{enumerate}
\end{lem}



The following structural result is due to Boissonnat, Guibas and 
Oudot~\cite[Lem.~4.3 \& 4.4]{boissonnat2009}.

\begin{lem}\label{lem-distance-point-on-M-with-sample}
    Let $L\subseteq \M$ be a $\epsilon$-sample of $\M$ with $\epsilon < \reach$, 
    and $\omega : L \rightarrow [0, \infty)$
    be a weight assignment with $\tilde{\omega} < \frac{1}{2}$.  
    \begin{enumerate}
        \item
            For all $p \in L$, $\omega(p) \leq 2 \tilde{\omega}\epsilon$.
        
        \item
            If $k$ is a non-negative integer and $\epsilon \leq \frac{\reach}{4}$, 
	    then, for all $x \in \M$ and $k \in \{0,\, 1\}$,
            the Euclidean distance between $x$ and its $k+1$-nearest weighted 
            neighbor in $L$ is at most $(1+2\tilde{\omega}+2k(1+3\tilde{\omega}))\epsilon$.  
        
    \end{enumerate}
\end{lem}





The following result is due to~\cite{boissonnat2012csdt}.

%is a direct consequence 
%of Lemma~\ref{lem-whitney-angle-bound}.

\begin{cor}\label{cor-angle-bound-simplex-tangent-space}
    Let $\sigma$ be a $k$-simplex with $k \leq m$ and the vertices of $\sigma$
    are on the submanifold $\M$. If $\sigma$ is $\sliverbnd$-good and
    $\Delta(\sigma) <  \reach$, then
    $$
        \sin \angle (\aff(\sigma), T_{p}\M) \leq \frac{\Delta(\sigma)}{\Gamma^{m}_{0} \reach}.
    $$
\end{cor}





%The following is from~\cite{boissonnat2012con.intrinsic}. This result is a
%variation of previous results from~\cite{niyogi2008, boissonnat2011tancplx}.

%\begin{lemma}[Tangent space variation]\label{lem-tangent-space-variation}
%    Let $x, \, y \in \M$ be such that $\dist{x}{y} \leq \frac{\reach}{4}$, and let
%    $\alpha$ be the angle between $T_{x}\M$ and $T_{y}\M$. Then,
%    $\sin \alpha < \frac{6\|x-y\|}{\reach}$.
%\end{lemma}



%The following lemma is due to~\cite{boissonnat2011cgl}.

%\begin{lemma}
%  \label{lem:flat.intersect}
%  Let $\tilde{c} \in \rdee$ be such that it has a unique closest point
%  $\hat{c}$ on $\man$ and $\norm{\tilde{c}- \hat{c}} \leq \mu \leq
%  \frac{\reach}{20}$.  Let $j \leq m = \dim\man$, and let $N$ be a
%  $(d-j)$-dimensional affine flat passing through $\tilde{c}$ such
%  that $\sin \angle (\normspace{\hat{c}}{\man}, N) \leq \frac{1}{4}$.
%%  with $\sin
%%  \alpha \leq \frac{1}{4}$.
%  Then there exists an $x \in N\cap \M$ such
%  that $\norm{\tilde{c} - x} \leq 4\mu$.
%\end{lemma}


%\subsection{Thick simplices}



\section{Almost normal flats intersecting submanifolds}
\label{appendix-normal-flats-intersecting-submanifolds}



\input{flat_intersect}








==> protection-1.tex <==



\section{Power protection and its consequences}

Let $\pts \subset \R^{d}$ be a point sample with $\dim \aff (\pts) = d$.
A simplex $\sigma \in \del_{\omega}(\pts)$ is {\em $\delta^{2}$-power
  protected}  at
$c \in \vor_{\omega}(\sigma)$
if for all $q \in L \setminus \sigma$ and $p \in \sigma$, then
$$
    \|q-c\|^{2} - \omega(q)^{2} > \|p-c\|^{2}-\omega(p)^{2} + \delta^{2}.
$$
The following result shows that power protecting 
$d$-simplices implies power protecting 
lower dimensional subsimplices as well.
\begin{lem}\label{thm-protection-lower-dim-simplices}
    	Let $\pts \subset \R^{d}$ be a set of points, and let 
	$\omega: \pts \rightarrow [0, \, \infty)$ be a weight
        assignment. In addition, let $p$ be a point of $\pts$  whose
        Voronoi cell
	$\vor_{\omega}(p)$ is bounded. Then, if all the $d$-simplices
	incident to $p$ in $\del_{\omega}(\pts)$
        are $\delta^{2}$-power
    	protected, with $\delta >0$, then
        any $j$-simplex incident to $p$ is 
	$\frac{\delta^{2}}{d-j+1}$-power protected.
\end{lem}
An interesting aspect of this result is the fact that the 
decay in power protection depends  linearly on the dimension 
of the ambient space. The proof of the theorem is done in the 
lifted $\R^{d+1}$ space where power protection 
translates into {\em vertical distance} of points in 
$\R^{d+1}$ from hyperplanes. See 
Appendix~\ref{appendix-proof-thm-protection-lower-dim-simplices}
for the full details.

Let $\alpha_{0} < \frac{1}{2}$ be an absolute constant, and 
$\Gamma_{0} < 1$ and $\delta_{0} < \alpha_{0}$ be paramters to the 
algorithm satisfying Eq.~\eqref{eqn-ineq-gamma-delta-alpha}. 
We define 
$\tilde{\alpha}_{0} \stackrel{\rm def}{=} \sqrt{\alpha^{2}_{0} - \delta^{2}_{0}}$.


Let $W \subset \M$ be an $\e$-sample of $\M$, $L \subset W$ 
a $\lambda$-net of $W$ with $\e \leq \lambda$, and 
$\omega: L \rightarrow [0, \infty)$ a weight assignment 
with $\tilde{\omega} \leq \tilde{\alpha}_{0}$ (to be defined later). 
A weight assignment $\xi: L \rightarrow [0, \infty)$ will be called an
{\em elementary weight perturbation} of 
$\omega$ ({\em ewp} for short)  if there exists $p \in L$ such that
$$
  \xi(p) \in \left[ \omega(p),\, \sqrt{\omega(p)^{2}+ \delta^{2}_{0}\lambda^{2}} 
  \right]
  \; \; \mbox{and} \; \; \xi(q) = \omega(q) 
  \;\; \mbox{if} \;\; q \in L \setminus p.
$$
% \begin{enumerate}
%  \item 
%     $\xi(p) \in [\omega(p), \, \sqrt{\omega(p)+ \delta^{2}_{0}\lambda^{2}}]$
%   ($\delta_{0}$ will be defined later).
%  \item
%     $\forall ~ q \in L \setminus p$, $\xi(q) = \omega(q)$.
% \end{enumerate}
We call the weight assignment $\omega: L \rightarrow [0, \infty)$
{\em stable} (resp.,  {\em locally stable at $p\in L$}) if for all ewp
$\xi$ of $\omega$, ${\rm K}_{\xi}(L)$
contains no $\Gamma_{0}$-slivers of dimension $\leq m+1$
(resp., no such slivers incident to $p$).

The main structural result in this section is the 
following theorem:
\begin{thm}\label{thm-output-weighted-rDT-eqal-wit}
%    Let $\Gamma_{0}$, $\delta_{0}$, and $\alpha_{0}< \frac{1}{2}$
%    be constants.
    Let $W \subset \M$ be an $\e$-sample of $\M$, $L \subset W$ be
    a $\lambda$-net of $W$ with $\e \leq \lambda$, and 
    $\omega: L \rightarrow [0, \infty)$ be a stable weight assignment.
%
%    weight assignment
%    satisfying the following conditions:
%    \begin{enumerate}
%     \item 
% 	$\tilde{\omega} \leq \tilde{\alpha}_{0} 
% 	\stackrel{{\rm def}}{=} \sqrt{\alpha^{2}_{0} - \delta^{2}_{0}}$.
% 
%      \item
% 	For all elementary weight perturbation (`ewp' for short)
% 	of $\xi: L \rightarrow [0, \infty)$ 
% 	of $\omega$, i.e. $\exists~ p \in L$ such that
% 	\begin{enumerate}
% 	 \item
% 	    $\xi(p)^{2} \in [\omega(p)^{2}, \omega(p)^{2} + \delta^{2}_{0}\lambda^{2}]$ and
% 
% 	 \item
% 	    for all $q \in L\setminus p$, $\xi(q) = \omega(q)$,
% 	\end{enumerate}
%	\vspace{3pt}
%	${\rm K}_{\xi}(L)$ contains no $\Gamma_{0}$-slivers
%	of dimension $\leq m+1$.
%    \end{enumerate}
    If 
    $$
      \lambda < \left\{ \frac{3\sin\theta_{0}}{2^{11}(m+1)},\,
      \frac{\sin\theta_{0}\Gamma^{m}_{0}}{2^{10}},\,
      \frac{\Gamma^{2m+1}_{0}}{24},\, \frac{\delta^{2}_{0}}{2^{15}(m+1)}
      \right\}\, \reach,
    $$
    and 
    $$
      \e < \frac{\lambda}{24}\left( \frac{\delta^{2}_{0}}{m+1} - \frac{2^{15}\lambda}{\reach}\right)
    $$
%    $$
%      \lambda < \left\{ \frac{\sin\theta_{0}}{2^{10}(m+1)}, 
%      \frac{\Gamma^{2m+1}_{0}}{2^{10}}, \frac{\delta^{2}_{0}}{2^{17}(m+1)}
%      \right\}\, \reach \; \; \mbox{and} \; \; 
%      \e < \frac{\lambda}{22}\left( \frac{\delta^{2}_{0}}{m+1} - \frac{2^{17}\lambda}{\reach}\right)
%    $$
%
%    $$
%      \lambda \leq XXX \;\;\; {\rm and} \;\;\; 
%      \e \leq YYY
%    $$
    then, 
    $$
      \del_{\omega}(L, T\M) = \wit_{\omega}(L, W).
    $$
    In addition, if $\lambda$ is sufficiently small, 
    $\wit_{\omega}(L, W)$ is homeomorphic and a close geometric approximation
    of $\M$.
  \end{thm}
   \begin{proof}[outline]
     We will give a brief outline of the proof. For full 
      details refer to Appendix~\ref{ssec-faces-inherit-protection}.
  
    Since $\omega$ is a stable weight assignment, 
    ${\rm K}_{\omega}(L)$ contains no $\Gamma_{0}$-slivers 
    of dimension $\leq m+1$ and $\lambda$ is sufficiently small, we can show
    the following:
    \begin{description}
     \item[P1]
	$\forall ~ \sigma \in \del_{\omega}(L, T\M)$ and $p \in \sigma$, 
	$\vor_{\omega}(\sigma) \cap T_{p}\M\neq\emptyset$
     
     \item[P2]
	the  simplices of $\del_{\omega}(L, T\M)$ 
	have dimension at most $m$, and the
	dimension of maximal simplices in ${\rm K}_{\omega}(L)$
	$\leq m$

     \item[P3]	
	$\wit_{\omega}(L, W) \subseteq \del_{\omega}(L, T\M)$
      
    \item[P4]
	 $\forall ~ \sigma \in {\rm K}_{\omega}(L)$,
	  $\angle (\aff\sigma, T_{p}\M) = O(\lambda)$ %, i.e., small


     \item[P5]
	$\del_{\omega}(L, T\M)$ is a faithful reconstruction of $\M$
      \end{description}
      P1, P2, P4 and P5 are direct consequences of results from
    from~\cite{cheng2005,boissonnat2009,boissonnat2011tancplx}.
%    P3 \framebox{add an argument}

%\highlight{
%\begin{proof}[of P3]
  We prove P3 by contradiction . Let $\sigma^{k} \in
  \wit_{\omega}(L,W)$ be a $k$-simplex with $\sigma^{k} \not\in
  \del_{\omega}(L, T\M)$ and $p$ a vertex of $\sigma^{k}$.  Using the sampling
  assumptions on $L$ and $W$, we can show that for all
  $\omega$-witness $w \in W$ of $\sigma^{k}$ or its subfaces, 
  $\|p-w\| = O(\lambda)$~\cite[Lem.~4.4]{boissonnat2009}.  
  This implies,
  from~\cite[Lem.~6]{giesen2004}, $d(w, T_{p}\M) =
  O(\frac{\lambda^{2}}{\reach})$. From~\cite[Thm.~4.1]{deSilva2008},
  we know that $\vor_{\omega}(\sigma^{k})$ intersects the convex hull
  of the $\omega$-witnesses of $\sigma^{k}$ and its
  subfaces. Let
  $c_{k} \in\vor_{\omega}(\sigma^{k})$ be a point in this
  intersection.  We have $d(c_{k}, T_{p}\M) =
  O(\frac{\lambda^{2}}{\reach})$ and, since $L$ is $\lambda$-sparse,
  $\|p-c_{k}\| = \Omega(\lambda)$.
  Therefore, using the sampling assumption on $\lambda$, we get
  $\frac{d(c_{k}, T_{p}\M)}{d(c_{k}, p)} = O(\frac{\lambda}{\reach}) <
  \sin \theta_{0}$. This implies
  that $\sigma^{k} \in {\rm K}_{\omega}(L)$.
  As $\angle (\aff\sigma^{k}, T_{p}\M)$ is small (property P4),
  $\exists~c_{k}'\in T_{p}\M$ such that the line segment $[c_{k},
  c_{k}']$ is orthogonal to $\sigma^{k}$ and $d(c_{k}, c_{k}') =
  O(\frac{\lambda^{2}}{\reach})$.  Again, as
  $\lambda$ is small, the line segment
  $[c_{k}, c_{k}']$ is contained in ${\rm K}_{\omega}(p)$. Since
  $\sigma^{k} \not \in \del_{\omega}(L, T\M)$, $\exists~ c_{k+1} \in
  [c_{k}, c_{k}']$ and a $(k+1)$-simplex $\sigma^{k+1}$ such that
  $c_{k+1} \in \vor_{\omega}(\sigma^{k+1})$ with $\sigma^{k} <
  \sigma^{k+1}$.  Therefore, $\sigma^{k+1} \in {\rm K}_{\omega}(L)$. 
  If  $k = m$,  we have reached a
  contradiction with property P2. 
%  Otherwise,
%  we apply the above  procedure to $\sigma^{k+1}$ and iterate until we
%  reach simplex $\sigma^{m+1}$ of dimension $m+1$, leading again to a
%  contradiction with property P2.
  Otherwise, using the facts that $\angle(\sigma^{k+1}, T_{p}\M)$ 
  is small, $d(c_{k+1}, T_{p}\M) = O(\frac{\lambda^{2}}{\reach})$
  and $d(p, c_{k+1}) = \Omega(\lambda)$, 
  we will find a $c'_{k+1} \in T_{p}\M$ such that 
  $[c_{k+1},c'_{k+1}] \in {\rm K}_{\omega}(p)$. Since 
  $\sigma^{k+1} \not\in {\rm K}_{\omega}(L)$, $\exists~c_{k+2} \in [c_{k+1},c'_{k+1}]$
  and $k+2$-simplex $\sigma^{k+2} \in {\rm K}_{\omega}(L)$
  such that $c_{k+2} \in \vor_{\omega}(\sigma^{k+2})$ and 
  $\sigma^{k+1}< \sigma^{k+2}$.
  Continuing this procedure of walking  
  on the Voronoi cell of the simplex from a point, like $c_{k+1}$, 
  in the intersection the Voronoi cell of the simplex and ${\rm K}_{\omega}(P)$ 
  towards $T_{p}\M$, we will get a sequence of points
  $$
    c_{k}, \dots, c_{m+1}
  $$
  and simplies 
  $$
    \sigma^{k} < \dots  < \sigma^{m+1}
  $$
  with $c_{j} \in \vor_{\omega}(\sigma^{j})\cap {\rm K}_{\omega}(p)$
  and $\sigma^{j} \in {\rm K}_{\omega}(L)$. We have now reached a contradiction 
  via property P2.
%
%  Otherwise, using the facts that
%   $\angle(\sigma^{k+1}, T_{p}\M)$ is small, $d(c_{k+1}, T_{p}\M) =
%   O(\frac{\lambda^{2}}{\reach})$ and $d(p, c_{k+1}) =
%   \Omega(\lambda)$, we will find a $c'_{k+1} \in T_{p}\M$ such that
%   $[c_{k+1},c'_{k+1}] \in {\rm K}^{\theta_{0}}(p)$. Since
%   $\sigma^{k+1} \not\in {\rm K}_{\omega}(L)$, $\exists~c_{k+2} \in
%   [c_{k+1},c'_{k+1}]$ and $k+2$-simplex $\sigma^{k+2} \in {\rm
%     K}_{\omega}(L)$ such that $c_{k+2} \in
%   \vor_{\omega}(\sigma^{k+2})$ and $\sigma^{k+1}< \sigma^{k+2}$.
%   Continuing this procedure of walking on a affine space orthogonal to
%   recent simplex from a point, like $c_{k+1}$, in the intersection the
%   Voronoi cell of the simplex and ${\rm K}^{\theta_{0}}(P)$ towards
%   $T_{p}\M$, we will get a sequence of points
% $$
%   c_{k}, \, c_{k+1}, \, \dots, c_{m}, \, c_{m+1}
% $$
% and simplies 
% $$
%   \sigma^{k} \subsetneq \sigma^{k} \subsetneq \dots  
%   \subsetneq \sigma^{m} \subsetneq \sigma^{m+1}
% $$
% with $c_{j} \in \vor_{\omega}(\sigma^{j})\cap {\rm K}^{\theta_{0}}(p)$
% and $\sigma^{j} \in {\rm K}_{\omega}(L)$. We have now reached a contradiction 
% via property P2.
%\qed
%\end{proof}
%}

  To complete the proof, we have to show $\del_{\omega}(L, T\M)
    \subseteq \wit_{\omega}(L, W)$.

%\begin{proof}[of $\del_{\omega}(L, T\M)
%    \subseteq \wit_{\omega}(L, W)$]
    We first show that all $m$-simplices in $\del_{\omega}(L, T\M)$
    are $\delta^{2}$-power protected on $T_{p}\M$, 
    where $\delta = \delta_{0}\lambda$.
    To reach a contradiction, let us assume that there exists a $m$-simplex $\sigma \in 
    \del_{\omega}(L, T\M)$ that is not power protected on $T_{p}\M$ for some 
    $p \in \sigma$. Then there exists  $c \in \vor_{\omega}(\sigma)\cap T_{p}\M$ 
    and $q \in L \setminus \sigma$ such that 
    $d(c,p^{\omega}) \geq d(c, q^{\omega}) - \delta^{2} $. Consider now the following 
    weight assignment:
%    $\xi(q) = \sqrt{\omega(q)^{2}+\beta^{2}}$,
%    and $\xi(x) = \omega(x)$ if $x \in L\setminus q$
    $$
          \xi(x) = \left\{
        \begin{array}{l l}
            \omega(x) & \quad \text{if $x\neq q$}\\
            \sqrt{\omega(q)^{2}+\beta^{2}} & \quad \text{if $x=q$}\\
        \end{array} \right.
    $$
    where $\beta^{2} = d(c,q^{\omega}) - d(c, p^{\omega})$. It is easy to 
    see that $\xi$ is an ewp of $\omega$ and $\tilde{\xi} < 1/2$.
    Let $\sigma' = q * \sigma$. Since $\lambda$ is sufficiently small,
    $\sigma'$ is a $\Gamma_{0}$-bad $(m+1)$-simplex.
    Broadly, the idea behind the proof
    is the following (see also the proofs of~\cite[Lem.~13]{cheng2005}
    and \cite[Lem.~4.9]{boissonnat2011tancplx}): the thickness of any
    $(m+1)$-simplex embedded in $\R^{m}$ is zero. Here  $\sigma '$ is
    a $(m+1)$-simplex embedded in $\R^d$ whose vertices belong to a
    small neighborhood of $\M \subset \R^d$. It follows that its
    thickness  is expected to be small.
%     and as the diameter of $\Delta(\sigma')$ is small
%     we would expect $\sigma'$ to have a small volume compared to its 
%     diameter and therefore be a `bad' simplex.
    Specifically, we prove that $\sigma'$ is $\Gamma_{0}$-bad, which 
    contradicts Property P2. %the fact that $\omega$ is a stable weight assignment.

    We now prove that all simplices (of all dimensions) in $\del_{\omega}(L, T\M)$ are
    $\frac{\delta^{2}}{m+1}$-power protected on $T_{p}\M$ for all $p \in
    \sigma$. To establish this result, we want to use
    Lemma~\ref{thm-protection-lower-dim-simplices} but we cannot use
    the theorem directly since it only holds
    for $d$-simplices of $\R^d$. To overcome this issue, we resort to 
%    Using property {\bf P1}, Lemma~2.2 of~\cite{boissonnat2010} and
%     Theorem~\ref{thm-protection-lower-dim-simplices}, we can prove
    Lemma~2.2 of~\cite{boissonnat2011tancplx} which states that 
    $\vor_{\omega}(L)\cap T_{p}\M$ is identical to
    a weighted Voronoi diagram $\vor_{\psi}(L')$  where
    $L'$ is the orthogonal projection of $L$ onto $T_{p}\M$, i.e.,
    $\vor_{\omega}(\sigma) \cap T_{p}\M = \vor_{\omega}(\sigma')$
    where $\sigma'$ is the projection of $\sigma$ onto $T_{p}\M$.
    Also we can prove, using P1, that $\delta^{2}$-power protection
    of a simplex $\sigma \in \del_{\omega}(L, T\M)$ incident to $p$ 
    on $T_{p}\M$
    implies 
    $\delta^{2}$-power protection of $\sigma' \in \del_{\psi}(L')$.
    Using this correspondance, we can show
    that all $m$-simplices incident to $p$ in $\del_{\psi}(L')$ are
    $\delta^{2}$-power protected since all the $m$-simplices incident to
    $p$ in $\del_{\omega}(L, T\M)$ are $\delta^{2}$-power protected on
    $T_{p}\M$.  
%    As we have now translated protection from
%    $m$-simplices in $\del_{\omega}(L, T\M)$ to $m$-simplices in a
%    weighted Delaunay complexes in $T_{p}\M$, a $m$-dimensional affine space, 
    We can now use
    Lemma~\ref{thm-protection-lower-dim-simplices}.  Using the
    bound on $\lambda$,  %sampling     bound on $L$ 
    we can show that $\vor_{\psi}(p) =
    \vor_{\omega}(p)\cap T_{p}\M$ is bounded,  
    see~\cite[Lem.~4.4]{boissonnat2011tancplx}.
    From
    Lemma~\ref{thm-protection-lower-dim-simplices}, we then get that all
    $j$-simplices in $\del_{\psi}(L')$
    incident to $p'$ are $\frac{\delta^{2}}{m+1}$-power
    protected. This result, together with the correspondence
    we have established with the power protection of 
    simplices incident to $p$ in $\del_{\psi}(L')$ with the
    power protection of 
    simplices incident to $p$ in $\del_{\omega}(L, T\M)$ on $T_{p}\M$,
    we deduce that all $j$-simplices  incident to $p$ in
    $\del_{\omega}(L, T\M)$ are $\frac{\delta^{2}}{m+1}$-power protected
    on $T_{p}\M$.  

    Let $\sigma$ be $\frac{\delta^{2}}{m+1}$-power protected
    at $c \in \vor_{\omega}(\sigma) \cap T_{p}\M$, where $p \in \sigma$.
    We can show that there exists $c' \in \M$, such that $\|c-c'\|$ is
    small compared to $\frac{\delta^{2}}{m+1}$ and the line passing 
    through $c$ and $c'$ is orthogonal to $\aff (\sigma )$. Using simple 
    triangle inequalities, we can prove that $\sigma$ is 
    $\Omega(\frac{\delta^{2}}{m})$-power protected at $c'$.
    
    As $W$ is an $\e$-sample of $\M$, we can find a $w \in W$
    such that $\|w-c'\| < \e$. Using the facts that $\e$ is much 
    smaller than $\delta^{2}= \delta^{2}_{0}\lambda^{2}$ and 
    $\sigma$ is $\Omega(\frac{\delta^{2}}{m})$-power protected at $c'$, 
    we get $w$ to be a witness of $\sigma$. Since $\sigma$ is an 
    arbitrary simplex of $\del_{\omega}(L, T\M)$, we have proved that
    $\del_{\omega}(L, T\M) \subseteq \wit_{\omega}(L, W)$. 
%    \qed
%    \end{proof}
\end{proof}







% 
% \textcolor{red}{DON'T READ THE REST OF THIS SECTION!}
% 
% 
% If 
% $\omega: L \rightarrow [0, \infty)$ 
% be a weight assignment with bounded relative amplitude,
% $\lambda$ sufficiently small, 
% and ${\rm K}^{\theta}_{\xi}(L)$ contains no slivers of dimension 
% $\leq m+1$ for all elementary perturbation $\xi$ (defined in 
% Theorem~\ref{thm-output-weighted-rDT-eqal-wit})
% of $\omega$, 
% then we prove that the $m$-simplices in 
% $\del_{\omega}(L, T\M)$ are power protected on the tangent spaces 
% of the vertices of simplices. 
% See, Lemma~\ref{lem-props-we-want-omega-to-satisfy}. Using, 
% Theorem~\ref{lem:dim-voronoi-protected-simplex}, we prove in 
% Lemma~\ref{lem-rDt-protected-M} that all the simplices of 
% $\del_{\omega}(L, \M)$ are power protected on the manifold. 
% Combining these results, we get for $\e$ sufficietly small 
% compared to the $\lambda$, 
% $\del_{\omega}(L, \M) \subseteq \wit_{\omega}(L, W)$.




% If $\lambda$ is small and ${\rm K}^{\theta}_{\omega}(\pts)$ has no slivers 
% of dimension $\leq m+1$ then 
%   \begin{enumerate}
%    \item
%       $\del_{\omega}(L, T\M) = \del_{\omega}(L, \M)$,
%     
%    \item	
%       $\forall ~\sigma \in \del_{\omega}(L, T\M)$ and 
%       $p \in \mathring{\sigma}$, 
%       $\vor_{\omega}(\sigma) \cap T_{p}\M \neq \emptyset$, 
% 
%   \item
%     dimension of maximal simplices in 
%     $\del_{\omega}(L, \M)$ is equal to $m$, and
% 
%   \item
%     $\wit_{\omega}(L, W) \subseteq \del_{\omega}(L, \M)$.
%   \end{enumerate}
%   See, Lemma~\ref{} from Appendix~\ref{}. This implies, from 
%   Lemma~\ref{} (in Appendix~\ref{}), that 
%   $\del_{\omega}(L, \M)$ is a faithful reconstruction of the manifold 
%   $\M$. 

%  So, the only thing left to show is that 
%  $\del_{\omega}(L, \M) \subseteq \wit_{\omega}(L, W)$.

% 
%   Combining all these results, we get the following theorem:
% Following definition will be important for the rest of this paper:
% \begin{definition}[Stable weight assignment]
%   We call a weight assignment $\omega: L \rightarrow [0, \infty)$
%   stable if for all ewp (defined in Theorem~\ref{thm-output-weighted-rDT-eqal-wit})
%   $\xi$ of $\omega$, ${\rm K}^{\theta_{0}}_{\xi}(L)$
%   contains no $\Gamma_{0}$-slivers of dimension $\leq m+1$.
% \end{definition} 
% 
% 
% 




==> protection.tex <==



\section{Power protection and its consequences}

Let $\pts \subset \R^{d}$ be a point sample with $\dim \aff (\pts) = d$.
A simplex $\sigma \in \del_{\omega}(\pts)$ is {\em $\delta^{2}$-power
  protected}  at
$c \in \vor_{\omega}(\sigma)$
if for all $q \in L \setminus \sigma$ and $p \in \sigma$, then
$$
    \|q-c\|^{2} - \omega(q)^{2} > \|p-c\|^{2}-\omega(p)^{2} + \delta^{2}.
$$
The following result shows that power protecting 
$d$-simplices implies power protecting 
lower dimensional subsimplices as well.
\begin{theorem}\label{thm-protection-lower-dim-simplices}
    	Let $\pts \subset \R^{d}$ be a set of points, and let 
	$\omega: \pts \rightarrow [0, \, \infty)$ be a weight
        assignment. In addition, let $p$ be a point of $\pts$  whose
        Voronoi cell
	$\vor_{\omega}(p)$ is bounded. Then, if all the $d$-simplices
	incident to $p$ in $\del_{\omega}(\pts)$
        are $\delta^{2}$-power
    	protected, with $\delta >0$, then
        any $j$-simplex incident to $p$ is 
	$\frac{\delta^{2}}{d-j+1}$-power protected.
\end{theorem}
An interesting aspect of this result is the fact that the 
decay in power protection depends  linearly on the dimension 
of the ambient space. The proof of the theorem is done in the 
lifted $\R^{d+1}$ space where power protection 
translates into {\em vertical distance} of points in 
$\R^{d+1}$ from hyperplanes.

Let $W \subset \M$ be an $\e$-sample of $\M$, $L \subset W$ 
a $\lambda$-net of $W$ with $\e \leq \lambda$, and 
$\omega: L \rightarrow [0, \infty)$ a weight assignment 
with $\tilde{\omega} \leq \tilde{\alpha}_{0}$ (to be defined later). 
A weight assignment $\xi: L \rightarrow [0, \infty)$ will be called an
{\em elementary weight perturbation} of 
$\omega$ ({\em ewp} for short)  if there exists $p \in L$ such that
\begin{enumerate}
 \item 
    $\xi(p) \in [\omega(p), \, \sqrt{\omega(p)+ \delta^{2}_{0}\lambda^{2}}]$
  ($\delta_{0}$ will be defined later).
 \item
    $\forall ~ q \in L \setminus p$, $\xi(q) = \omega(q)$.
\end{enumerate}
We call the weight assignment $\omega: L \rightarrow [0, \infty)$
{\em stable} (resp.,  {\em locally stable at $p\in L$}) if for all ewp
$\xi$ of $\omega$, ${\rm K}_{\xi}(L)$
contains no $\Gamma_{0}$-slivers of dimension $\leq m+1$
(resp., incident at $p$).

The main structural result in this section is the 
following theorem:
  \begin{theorem}\label{thm-output-weighted-rDT-eqal-wit}
    Let $\Gamma_{0}$, $\delta_{0}$, and $\alpha_{0}< \frac{1}{2}$
    be constants.
    Let $W \subset \M$ be an $\e$-sample of $\M$, $L \subset W$ be
    a $\lambda$-net of $W$ with $\e \leq \lambda$, and 
    $\omega: L \rightarrow [0, \infty)$ be a stable weight assignment.
%
%    weight assignment
%    satisfying the following conditions:
%    \begin{enumerate}
%     \item 
% 	$\tilde{\omega} \leq \tilde{\alpha}_{0} 
% 	\stackrel{{\rm def}}{=} \sqrt{\alpha^{2}_{0} - \delta^{2}_{0}}$.
% 
%      \item
% 	For all elementary weight perturbation (`ewp' for short)
% 	of $\xi: L \rightarrow [0, \infty)$ 
% 	of $\omega$, i.e. $\exists~ p \in L$ such that
% 	\begin{enumerate}
% 	 \item
% 	    $\xi(p)^{2} \in [\omega(p)^{2}, \omega(p)^{2} + \delta^{2}_{0}\lambda^{2}]$ and
% 
% 	 \item
% 	    for all $q \in L\setminus p$, $\xi(q) = \omega(q)$,
% 	\end{enumerate}
%	\vspace{3pt}
%	${\rm K}_{\xi}(L)$ contains no $\Gamma_{0}$-slivers
%	of dimension $\leq m+1$.
%    \end{enumerate}
    If 
$$
  \lambda < \left\{ \frac{\sin\theta_{0}}{2^{10}(m+1)}, 
  \frac{\Gamma^{2m+1}_{0}}{2^{10}}, \frac{\delta^{2}_{0}}{2^{17}(m+1)}
  \right\}\, \reach \; \; \mbox{and} \; \; 
  \e < \frac{\lambda}{22}\left( \frac{\delta^{2}_{0}}{m+1} - \frac{2^{17}\lambda}{\reach}\right)
$$
%    $$
%      \lambda \leq XXX \;\;\; {\rm and} \;\;\; 
%      \e \leq YYY
%    $$
    then, 
    $\del_{\omega}(L, T\M) = \wit_{\omega}(L, W)$.
In addition, if $\lambda$ is sufficiently small, 
    $\wit_{\omega}(L, W)$ is homeomorphic and a close geometric approximation
    of $\M$.
  \end{theorem}
  \begin{proof}[Brief outline]
    We will give a brief outline of the proof of 
    Theorem~\ref{thm-output-weighted-rDT-eqal-wit}.
    
    Since ${\rm K}_{\omega}(L)$ contains no $\Gamma_{0}$-slivers 
    of dimension $\leq m+1$ and $\lambda$ is sufficiently small, we can show
    the following:
    \begin{description}
     \item[P1]
	$\forall ~ \sigma \in \del_{\omega}(L, T\M)$ and $p \in \sigma$, 
	$\vor_{\omega}(\sigma) \cap T_{p}\M$
     
     \item[P2]
	dimension of maximal simplices in $\del_{\omega}(L, T\M)$ is 
	equal to $m$, and 
	dimension of maximal simplices in ${\rm K}_{\omega}(L)$
	$\leq m$

     \item[P3]	
	$\wit_{\omega}(L, W) \subseteq \del_{\omega}(L, T\M)$
      
    \item[P4]
	 $\forall ~ \sigma \in {\rm K}_{\omega}(L)$,
	  $\angle (\aff\sigma, T_{p}\M) = O(\lambda)$, i.e., small


     \item[P5]
	$\del_{\omega}(L, T\M)$ is a faithful reconstruction of $\M$
      \end{description}
      P1, P2, P4 and P5 are direct consequences of results from
    from~\cite{cheng2005,boissonnat2009,boissonnat2011tancplx}.
    P3 \framebox{add an argument}

\textcolor{blue}{
%We will give a outline of the proof of P3. 
We prove P3 by contradiction . Let 
$\sigma^{k} \in \wit_{\omega}(L,W)$ be a $k$-simplex with 
$\sigma^{k} \not\in \del_{\omega}(L, T\M)$ and $p$ a vertex of $\sigma^{k}$. 
Without loss of generality, we assume $k\leq m$.
Using the sampling assumptions 
on $L$ and $W$, we can show
that for all $\omega$-witness $w \in W$ of $\sigma^{k}$, $\|p-w\| = O(\lambda)$.
See~\cite[Lem.~4.4]{boissonnat2009}.
This implies, from~\cite[Lem.~6]{giesen2004}, 
$d(w, T_{p}\M) = O(\frac{\lambda^{2}}{\reach})$. From~\cite[Cor.~7.6]{deSilva2008}, 
we know that $\vor_{\omega}(\sigma^{k})$ intersects the convex hull of the 
$\omega$-witnesses of $\sigma^{k}$ and its subfaces. Lets 
$c_{k} \in\vor_{\omega}(\sigma^{k})$
be a point in this intersection. 
This implies $d(c_{k}, T_{p}\M) = O(\frac{\lambda^{2}}{\reach})$, and
since $L$ is $\lambda$-sparse, we can show
that $\|p-c_{k}\| = \Omega(\lambda)$.
Therefore, %using the sampling assumption on $\lambda$, we get 
$\frac{d(c_{k}, T_{p}\M)}{d(c_{k}, p)} = 
O(\frac{\lambda}{\reach}) < \sin \theta_{0}$. This implies 
$\sigma^{k} \in {\rm K}_{\omega}(L)$. 
As $\angle (\aff\sigma^{k}, T_{p}\M)$ is small (property P4), 
$\exists~c_{k}'\in T_{p}\M$ such that the line segment 
$[c_{k}, c_{k}']$ is orthogonal to $\sigma^{k}$ and 
$d(c_{k}, c_{k}') = O(\frac{\lambda^{2}}{\reach})$.
Again, using the fact that $\lambda$ is sufficiently small we can show 
that the line segment $[c_{k}, c_{k}']$ is contained in 
${\rm K}^{\theta_{0}}(p)$. Since $\sigma^{k} \not \in \del_{\omega}(L, T\M)$, 
$\exists~ c_{k+1} \in [c_{k}, c_{k}']$ and a $k+1$-simplex $\sigma^{k+1}$
such that
$c_{k+1} \in \vor_{\omega}(\sigma^{k+1})$ with $\sigma^{k} < \sigma^{k+1}$. 
Therefore we have $\sigma^{k+1} \in {\rm K}_{\omega}(L)$, and if $k+1 = m+1$
we have reached a contradiction with property P2. 
Otherwise, using the facts that $\angle(\sigma^{k+1}, T_{p}\M)$ 
is small, $d(c_{k+1}, T_{p}\M) = O(\frac{\lambda^{2}}{\reach})$
and $d(p, c_{k+1}) = \Omega(\lambda)$, 
we will find a $c'_{k+1} \in T_{p}\M$ such that 
$[c_{k+1},c'_{k+1}] \in {\rm K}^{\theta_{0}}(p)$. Since 
$\sigma^{k+1} \not\in {\rm K}_{\omega}(L)$, $\exists~c_{k+2} \in [c_{k+1},c'_{k+1}]$
and $k+2$-simplex $\sigma^{k+2} \in {\rm K}_{\omega}(L)$
such that $c_{k+2} \in \vor_{\omega}(\sigma^{k+2})$ and 
$\sigma^{k+1}< \sigma^{k+2}$.
Continuing this procedure of walking  
on a affine space orthogonal to recent simplex from a point, like $c_{k+1}$, 
in the intersection the Voronoi cell of the simplex and ${\rm K}^{\theta_{0}}(P)$ 
towards $T_{p}\M$, we will get a sequence of points
$$
  c_{k}, \, c_{k+1}, \, \dots, c_{m}, \, c_{m+1}
$$
and simplies 
$$
  \sigma^{k} \subsetneq \sigma^{k} \subsetneq \dots  
  \subsetneq \sigma^{m} \subsetneq \sigma^{m+1}
$$
with $c_{j} \in \vor_{\omega}(\sigma^{j})\cap {\rm K}^{\theta_{0}}(p)$
and $\sigma^{j} \in {\rm K}_{\omega}(L)$. We have now reached a contradiction 
via property P2.
}



    It remains to prove that the inclusion $\del_{\omega}(L, T\M)
    \subseteq \wit_{\omega}(L, W)$.

    We will now show that all the $m$-simplices in $\del_{\omega}(L, T\M)$
    are $\delta^{2}$-power protected, where $\delta = \delta_{0}\lambda$.
    To reach a contradiction, let us assume that there exists a $m$-simplex $\sigma \in 
    \del_{\omega}(L, T\M)$ that is not power protected on $T_{p}\M$ for some 
    $p \in \sigma$. Then there exists  $c \in \vor_{\omega}(\sigma)\cap T_{p}\M$ 
    and $q \in L \setminus \sigma$ such that 
    $d(c,p^{\omega}) \geq d(c, q^{\omega}) - \delta^{2} $. Consider now the following 
    weight assignment
    $$
      \xi(q) = \sqrt{\omega(q)^{2}+\beta^{2}},\;\;
      {\rm  and}\;\; \xi(x) = \omega(x) \;\;{\rm  if}\;\; x \in L\setminus q 
    $$
%    $$
%          \xi(x) = \left\{
%        \begin{array}{l l}
%            \omega(x) & \quad \text{if $x\neq q$}\\
%            \sqrt{\omega(q)^{2}+\beta^{2}} & \quad \text{if $x=q$}\\
%        \end{array} \right.
%    $$
    where $\beta^{2} = d(c,q^{\omega}) - d(c, p^{\omega})$. It is easy to 
    see that $\xi$ is an ewp of $\omega$,  $\tilde{\xi} <
    \frac{1}{2}$. Let
    $\sigma' = q * \sigma$. Since $\lambda$ is sufficiently small,
    $\sigma'$ is a $\Gamma_{0}$-bad $(m+1)$-simplex.
    Broadly, the idea behind the proof
    is the following (see also the proofs of~\cite[Lem.~13]{cheng2005}
    and \cite[Lem.~4.9]{boissonnat2011tancplx}): the thickness of any
    $(m+1)$-simplex embedded in $\R^{m}$ is zero. Here  $\sigma '$ is
    a $(m+1)$-simplex embedded in $\R^d$ whose vertices belong to a
    small neighborhood of $\M \subset \R^d$. It follows that its
    thickness  is expected to be small.
%     and as the diameter of $\Delta(\sigma')$ is small
%     we would expect $\sigma'$ to have a small volume compared to its 
%     diameter and therefore be a `bad' simplex.
    Specifically, we prove that $\sigma'$ is $\Gamma_{0}$-bad, which 
    contradicts the fact that $\omega$ is a stable weight assignment.


    Using property {\bf P1}, Lemma~2.2 of~\cite{boissonnat2010} and
    Theorem~\ref{thm-protection-lower-dim-simplices}, we can prove
    that all simplices in $\del_{\omega}(L, T\M)$ are
    $\frac{\delta^{2}}{m+1}$-power protected on $T_{p}\M$ for all $p \in
    \sigma$. To establish this result, we first use
    Lemma~2.2 of~\cite{boissonnat2011tancplx} which states that the
    restricted Voronoi $\vor_{\omega}(L)\cap T_{p}\M$ is identical to
    a weighted Voronoi diagram $\vor_{\psi}(L')$  where
    $L'$ is the orthogonal projection of $L$ onto $T_{p}\M$.  This
    implies that if a simplex $\sigma$ of
    $\del_{\omega}(L, T\M)$ is incident to $p$, its orthogonal
    projection $\sigma'$ onto $T_p\M$ is incident to $p$ in
    $\del_{\psi}(L')$. Using this framework,
    we can show
    that all $m$-simplices incident to $p$ in $\del_{\psi}(L')$ are
    $\delta^{2}$-power protected since all the simplices incident to
    $p$ in $\del_{\omega}(L, T\M)$ are $\delta^{2}$-power protected on
    $T_{p}\M$.  As we have now translated protection from
    $m$-simplices in $\del_{\omega}(L, T\M)$ to $m$-simplices in a
    weighted Delaunay complexes in $m$-dimensional affine space, we
    will be able to use
    Theorem~\ref{thm-protection-lower-dim-simplices}.  Using sampling
    bound on $L$ we can show that $\vor_{\psi}(p')$ ($ =
    \vor_{\omega}(p)\cap T_{p}\M$) where $p'$ is a projection of $p$
    onto $T_{p}\M$, see~\cite[Lem.~4.4]{boissonnat2011tancplx}.  From
    Theorem~\ref{thm-protection-lower-dim-simplices}, we get that all
    $j$-simplices incident to $p'$ are $\frac{\delta^{2}}{m+1}$-power
    protected. From the identity 
    $\vor_{\psi}(L')=\vor_{\omega}(L)\cap T_{p}\M$ and Property
    P1,  we deduce that all $j$-simplices  incident to $p$ in
    $\del_{\omega}(L, T\M)$ are $\frac{\delta^{2}}{m+1}$-power protected
    on $T_{p}\M$.  

    Let $\sigma$ be $\frac{\delta^{2}}{m+1}$-power protected
    at $c \in \vor_{\omega}(\sigma) \cap T_{p}\M$, where $p \in \sigma$.
    We can show that there exists $c' \in \M$, such that $\|c-c'\|$ is
    small compared to $\frac{\delta^{2}}{m+1}$ and the line passing 
    through $c$ and $c'$ is orthogonal to $\aff (\sigma )$. Using simple 
    triangle inequalities, we can prove that $\sigma$ is 
    $\Omega(\frac{\delta^{2}}{m})$-power protected at $c'$.
    
    As $W$ is an $\e$-sample of $\M$, we can find a $w \in W$
    such that $\|w-c'\| < \e$. Using the facts that $\e$ is much 
    smaller than $\delta^{2}= \delta^{2}_{0}\lambda^{2}$ and 
    $\sigma$ is $\Omega(\frac{\delta^{2}}{m})$-power protected at $c'$, 
    we get $w$ to be a witness of $\sigma$. Since $\sigma$ is an 
    arbitrary simplex of $\del_{\omega}(L, T\M)$, we have proved that
    $\del_{\omega}(L, T\M) \subseteq \wit_{\omega}(L, W)$. 
  \qed
  \end{proof}








% 
% \textcolor{red}{DON'T READ THE REST OF THIS SECTION!}
% 
% 
% If 
% $\omega: L \rightarrow [0, \infty)$ 
% be a weight assignment with bounded relative amplitude,
% $\lambda$ sufficiently small, 
% and ${\rm K}^{\theta}_{\xi}(L)$ contains no slivers of dimension 
% $\leq m+1$ for all elementary perturbation $\xi$ (defined in 
% Theorem~\ref{thm-output-weighted-rDT-eqal-wit})
% of $\omega$, 
% then we prove that the $m$-simplices in 
% $\del_{\omega}(L, T\M)$ are power protected on the tangent spaces 
% of the vertices of simplices. 
% See, Lemma~\ref{lem-props-we-want-omega-to-satisfy}. Using, 
% Theorem~\ref{lem:dim-voronoi-protected-simplex}, we prove in 
% Lemma~\ref{lem-rDt-protected-M} that all the simplices of 
% $\del_{\omega}(L, \M)$ are power protected on the manifold. 
% Combining these results, we get for $\e$ sufficietly small 
% compared to the $\lambda$, 
% $\del_{\omega}(L, \M) \subseteq \wit_{\omega}(L, W)$.




% If $\lambda$ is small and ${\rm K}^{\theta}_{\omega}(\pts)$ has no slivers 
% of dimension $\leq m+1$ then 
%   \begin{enumerate}
%    \item
%       $\del_{\omega}(L, T\M) = \del_{\omega}(L, \M)$,
%     
%    \item	
%       $\forall ~\sigma \in \del_{\omega}(L, T\M)$ and 
%       $p \in \mathring{\sigma}$, 
%       $\vor_{\omega}(\sigma) \cap T_{p}\M \neq \emptyset$, 
% 
%   \item
%     dimension of maximal simplices in 
%     $\del_{\omega}(L, \M)$ is equal to $m$, and
% 
%   \item
%     $\wit_{\omega}(L, W) \subseteq \del_{\omega}(L, \M)$.
%   \end{enumerate}
%   See, Lemma~\ref{} from Appendix~\ref{}. This implies, from 
%   Lemma~\ref{} (in Appendix~\ref{}), that 
%   $\del_{\omega}(L, \M)$ is a faithful reconstruction of the manifold 
%   $\M$. 

%  So, the only thing left to show is that 
%  $\del_{\omega}(L, \M) \subseteq \wit_{\omega}(L, W)$.

% 
%   Combining all these results, we get the following theorem:
% Following definition will be important for the rest of this paper:
% \begin{definition}[Stable weight assignment]
%   We call a weight assignment $\omega: L \rightarrow [0, \infty)$
%   stable if for all ewp (defined in Theorem~\ref{thm-output-weighted-rDT-eqal-wit})
%   $\xi$ of $\omega$, ${\rm K}^{\theta_{0}}_{\xi}(L)$
%   contains no $\Gamma_{0}$-slivers of dimension $\leq m+1$.
% \end{definition} 
% 
% 
% 




==> stability-power-protection-weighted-Delaunay.tex <==


%\section{Stability under perturbation}
%\label{sec-stability-weighted-Delaunay}


\section{Stability of weighted circumcentres}
\label{sec-stability-weighted-circumcentres}

Let $\pts = \{ p_{0}, \, \dots, \, p_{n-1}\} \subset U \subset \reel^{d}$, and 
$\omega: \pts \rightarrow \reel^{\geq 0}$ be a weight assignment. For a metric
$D : U \times U \rightarrow \R^{\geq 0}$, we can define 
{\em $\omega$-weighted squared distance} wrt $D(.,\, .)$ as 
$D(p^{\omega}, x) = D(p,x)^{2} - \omega(p)^{2}$.


%\begin{itemize}
% \item 
% $\mathrm{D}_{d}(p^{\omega}, x) \stackrel{\rm def}{=} \dist{p}{x}^{2} - \omega(p)^{2}$
% 
% \item
% $\distreel{d}{p^{\omega}}{x} \stackrel{\rm def}{=} \|p-x\|^{2} - \omega(p)^{2}$
%\end{itemize}


\begin{definition}
 Let $\omega: \{p_{0}, \dots, p_{k}\} \rightarrow [0,\infty)$.
 A $\xi^{2}$-weighted Euclidean center
 $\omega$-center for a simplex $\sigma = [p_{0}, \dots, p_{k}] \subset \reel^{d}$
 is a point $x$ that satisfies 
 \begin{equation}
    \mid d(p_{i}^{\omega}, x) - d(p_{j}^{\omega},x) \mid \; \leq \; \xi^{2} \quad \forall\, 
    p_{i}, \, p_{j} \in \sigma.
 \end{equation}
\end{definition}

The following result shows that approximate weighted center is close to 
the actual weighted center for non-degenerate simplex. The proof is same as the proof 
of~\cite[Lemma~4.1]{boissonnat2012sdt}.
\begin{lem}\label{lem-distance-of-relaxed-centre}
 If $\sigma = [p_{0}, \dots, p_{k}] \subset \reel^{m}$ is a non-degenerate $k$-simplex, 
 $\omega: \sigma \rightarrow [0, \infty)$ be a weight function, and 
 $x \in \reel^{m}$ is a $\xi^{2}$-weighted Euclidean
 $\omega$-center of $\sigma$, then 
 \begin{equation}
  \|C_{\omega}(\sigma) - x\| \leq \frac{\xi^{2}}{2 \Upsilon(\sigma) \Delta(\sigma)}.
 \end{equation}
\end{lem}
Using Lemma~\ref{lem-distance-of-relaxed-centre}, we can prove the stability of 
weighted Euclidean circumcentre under perturbation of the weight assignments:

\begin{lem}[Stab. of w. centre under weight pert.]
\label{lem-stability-weighted-circumcentre-weight-pert}
 If $\sigma = [p_{0}, \dots, p_{k}] \subset \reel^{m}$ is a non-degenerate $k$-simplex, 
 and
 $\omega_{1}, \, \omega_{2} : \sigma \rightarrow [0, \infty)$ be a weight functions
 with $| \omega_{1}(p_{i})^{2} - \omega_{2}(p_{i})^{2} | \leq \rho^{2}$, then 
 \begin{equation}
  \|C_{\omega_{1}}(\sigma) - C_{\omega_{2}}(\sigma)\| \leq \frac{\rho^{2}}{\Upsilon(\sigma) \Delta(\sigma)}.
 \end{equation}
\end{lem}



\begin{lem}
[Stab. of w. centre under metric pert.]
\label{lem-stab-weighted-center-metric-pert}
 Let $U \subset \reel^{m}$, and $D : U \times U \rightarrow \reel$ be a continuous metric 
 with respect to the topology defined by Euclidean $2$-norm $d = \|\|$, and such that for any 
 $x, \, y \in U$ with $d(x, y) < 2C \epsilon$
 where $C \geq 1$ is a constant, we have 
 $\mid \dist{x}{y}^{2} - D(x,y)^{2} \mid \leq \rho^{2}$, with 
 $$
    \frac{2\rho^{2}}{\Upsilon_{0} \mu_{0}} \leq \epsilon^{2}.
 $$
 Let $\omega: \sigma = \{ p_{0}, \dots, p_{m}\} \rightarrow [0, \infty)$ be weight 
 function, $\sigma$ is a $\Upsilon_{0}$-thick $m$-simplex with $R_{\omega}(\sigma) < C\epsilon$,
 and $L(\sigma) \geq \mu_{0}\epsilon$, such that $d(p_{i}, \partial U) \geq 2C\epsilon$, 
 then there is a point 
 $$
  x \in B(c, \eta)\quad \mbox{where} \quad \eta = \frac{2\rho^{2}}{\Upsilon_{0}\mu_{0}\epsilon}
  \quad c = C_{\omega}(\sigma)
 $$
 and such that $D(p^{\omega}_{i},x) = D(p^{\omega}_{j},x)$ 
 for all $p_{i},\, p_{j} \in \sigma$.
\end{lem}
The proof of Lemma~\ref{lem-stab-weighted-center-metric-pert} follows along the same lines 
as the proof of \cite[Lem.~4.4]{boissonnat2012sdt}. We will give the outline of the proof 
in this section. 


Let $B = B(C_{\omega}(\sigma), \eta)$, and 
$f_{e}, \; f : \overline{B} \rightarrow \reel^{m}$ be two functions defined as follows:
\begin{eqnarray*}
 f_{e}(x) &=& \left( d(p_{1}^{\omega},x) - 
 d(p_{0}^{\omega},x), \,\dots, 
 \,d(p_{m}^{\omega},x) - d(p_{0}^{\omega},x) \right) \\
 f(x) &=& \left( D(p_{1}^{\omega},x) - 
 D(p_{0}^{\omega},x), \,\dots, 
 \, D(p_{m}^{\omega},x) - D(p_{0}^{\omega},x) \right)  
\end{eqnarray*}
The goal is to show $f^{-1}(0) \neq \emptyset$. 

We can show the following:
\begin{description}
 \item[Part-1.]
 There is a homotopy $F: \overline{B} \times [0,\, 1] \rightarrow$ between $f_{e}(x) = F(x,0)$
 and $f(x) = F(x,1)$ with $F(x,t) \neq 0$ for all $x \in \partial \, \overline{B}$ and 
 $\forall \, t \in [0,\, 1]$. \textcolor{blue}{We need Lemma~\ref{lem-distance-of-relaxed-centre}.}
 
 \item[Part-2.]
 $c = C_{\omega}(\sigma)$ is a regular value of the function $f_{e}(x)$, with 
 $| \mathrm{det} J (f_{e}(c)) | = m! \vol(\sigma)$.
 
\end{description}


\textcolor{red}{
Lemma~\ref{lem-stab-weighted-center-metric-pert} 
now follows from a consideration of the
degree of the mappings $f$ and $f_e$ relative to zero. The
\defn{degree} of a smooth map $g: \close{B} \to \rem$ at a regular
point $p \in g(B)$ is defined by
\begin{equation*}
  \deg (g,p,B) = \sum_{x \in g^{-1}(p)} \sgn \det J(g)_x \, ,
\end{equation*}
where $J(g)_x$ is the Jacobian matrix of $g$ at $x$.
The exposition by Dancer~\cite{dancer2000} is a good reference for the
degree of maps from manifolds with boundary. It is shown that the
definition of $\deg(g,p,B)$ extends to continuous maps $g$ that are
not necessarily differentiable. If $h: \close{B} \to \rem$ is
homotopic to $g$ by a homotopy $H: \close{B} \times [0,1] \to \rem$
such that $H(x,t) \neq p$ for all $t \in [0,1]$, and $x \in \bdry{B}$,
then $\deg (g,p,B) = \deg(h,p,B)$.}

\textcolor{red}{
Since $f_e^{-1}(0) = \{ \circcentre{\splxs} \}$, it follows from
\Lemref{lem:fe.regular} that $\deg(f_e,0,B) = \pm 1$. Then
\Lemref{lem:fef.homotopic} implies $\deg(f,0,B) = \deg(f_e,0,B)$,
and since this is nonzero, it must be that $f^{-1}(0) \neq \emptyset$.
The demonstration of \Lemref{lem:metric.cc.pert} is complete.
}


Combining Lemmas~\ref{lem-distance-of-relaxed-centre} and \ref{lem-stab-weighted-center-metric-pert}, 
we get the following theorem:
\begin{thm}
[Stab. of w. centre under weight and metric pert.]
\label{thm-stab-weighted-center-metric-weight-pert}
 Let $U \subset \reel^{m}$, and $D : U \times U \rightarrow \reel$ be a continuous metric 
 with respect to the topology defined by Euclidean $2$-norm $d = \|\|$, and such that for any 
 $x, \, y \in U$ with $d(x, y) < 2C \epsilon$
 where $C \geq 1$ is a constant, we have 
 $\mid \dist{x}{y}^{2} - D(x,y)^{2} \mid \leq \rho_{1}^{2}$, with 
 $$
    \frac{2\rho^{2}_{1}}{\Upsilon_{0} \mu_{0}} \leq \epsilon^{2}.
 $$
 Let $\omega_{1}, \, \omega_{2}: \sigma = \{ p_{0}, \dots, p_{m}\} \rightarrow [0, \infty)$ 
 be weight assignments with 
 $$
  | \omega_{1}(p_{i})^{2} - \omega_{2}(p_{i})^{2}| \leq \rho_{2}^{2}, \quad \forall \, p_{i} \in \sigma.
 $$
 The simplex
 $\sigma \subset U$ is a 
 $\Upsilon_{0}$-thick $m$-simplex with $R_{\omega_{i}}(\sigma) < C\epsilon$ for 
 all $i \in \{ 1, \, 2\}$,
 and $L(\sigma) \geq \mu_{0}\epsilon$, such that $d(p_{i}, \partial U) \geq 2C\epsilon$, 
 then there is a point 
 $$
  x \in B(c, \eta)\quad \mbox{where} \quad \eta = \frac{2\rho_{1}^{2}+\rho_{2}^{2}}{\Upsilon_{0}\mu_{0}\epsilon}
  \; \mbox{and} \; c = C_{\omega_{1}}(\sigma)
 $$
 and such that $D(p^{\omega_{2}}_{i},x) = D(p^{\omega_{2}}_{j},x)$ 
 for all $p_{i},\, p_{j} \in \sigma$.
\end{thm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

